Search for chargino-neutralino production in p-pbar collisions at 1.96 TeV with high pT leptons

We present a search for the associated production of charginos and neutralinos in p-pbar collisions at 1.96 TeV. The data were collected at the Collider Detector at Fermilab (CDF II) and correspond to integrated luminosities between 0.7 and 1.0 fb-1. We look for final states with one high pT electron or muon, and two additional leptons. Our results are consistent with the standard model expectations, and we set limits on the cross section as a function of the chargino mass in three different supersymmetric scenarios. For a specific MSSM scenario with no slepton mixing we set a 95 % C.L. limit at 151 GeV/c^2.

==> abstract.tex <==
\begin{abstract}
We present a search for the associated production of charginos
and neutralinos in $\rm {p \bar p}$ collisions at $\sqrt{s}$ = 1.96 TeV. The data were collected at the Collider Detector at Fermilab (CDF II)
and correspond to integrated luminosities between 0.7 and 1.0 fb$^{-1}$.
%depending on the search channel. 
We look
for final states with one high-\pt\  electron or muon, and two additional
leptons.
Our
results are consistent with the standard model expectations, and we
set limits on the cross section as a function of the chargino mass  in 
three different supersymmetric scenarios. For a specific MSSM scenario with no slepton mixing we 
set a 95\% C.L. limit at 151 GeV/$c^2$.
\end{abstract}

